Modelling and Optimising GaAs/Al(x)Ga(1-x)As Multiple Quantum Well Solar Cells

The quantum well solar cell (QWSC) is a p - i - n solar cell with quantum wells in the intrinsic region. Previous work has shown that QWSCs have a greater open circuit voltage (Voc) than would be provided by a cell with the quantum well effective bandgap. This suggests that the fundamental efficiency limits of QWSCs are greater than those of single bandgap solar cells. The following work investigates QWSCs in the GaAs/AlxGa1-xAs materials system. The design and optimisation of a QWSC in this system requires studies of the voltage and current dependencies on the aluminium fraction. QWSCs with different aluminium fractions have been studied and show an increasing Voc with increasing barrier aluminium composition. The QE however decreases with increasing aluminium composition. We develop a model of the QE to test novel QWSC designs with a view to minimising this problem. This work concentrates on two design changes. The first deals with com- positionally graded structures in which the bandgap varies with position. This bandgap variation introduces an quasi electric field which can be used to increase minority carrier collection in the low efficiency p and n layers. This technique also increases the light flux reaching the highly efficient depletion regions. The second design change consists of coating the back of the cell with a mirror to exploit the portion of light which is not absorbed on the first pass. A model of the QE of compositionally graded QWSC solar cells with back surface mirrors is developed in order to analyse the effect of these design changes. These changes are implemented separately in a number of QWSC designs and the resulting experimental data compared with the model. An optimised design is then presented.

==> acknow.tex <==
\begin{acknowledgements}

The work in this thesis could not have happened without the
support of a multitude of people. Keith Barnham has been a
tireless source of encouragement and ideas over the years.
And endless thanks to Jenny Nelson for always knowing what was
wrong with models, and helping with encyclopaedic knowledge,
and being there to recommend films, or have them recommended!
Then there are all those who have passed through here, or
are still here, including Jenny Barnes, Ian Ballard, Alex
Zachariou, Paul Griffin, Ernest Tsui and Ned, whom I thank
for coffee times.

Next come the people who actually produced the solar cells in
this thesis. Christine Roberts was always ready to answer
constant questions about MBE machines and AlGaAs. John
Roberts' produced the grade which worked
first time, and was full of suggestions for new material tests. 
Malcolm Pate produced innumerable devices over the years, including
the wafer squashed in the post!

Then there are collaborators overseas. Antonio Marti helped me
take some measurements which can't be fitted in. Two hundred pages
is quite enough! And Rosa Maria Fernadez Reyna in Madrid, who
explained them to me and showed me one of the best cinemas I
know, and one of the nicest cafes too.

Enrique Gr\"unbaum took TEM measurements which helped explain one
of the more mystifying samples in this project, along with SIMS
measurements by Federico Caccavale. The latter were due to Max Mazzer 
who arranged the SIMS measurements in Padua, and always 
had ideas for everything, including jazz!

And thanks to all the people who have made daily life about the
department more interesting, such as Jean Leveratt for chats on 
level 8 at lunchtimes and solutions to all sorts of problems, and
to Betty Moynihan for help with the technicalities of writing up
on level 3.

As for finance, I thank the Greenpeace Trust who made the project
possible, and who enabled me to go to the Solar World Congress.

Finally, there all the people I have known, or got to know over
the years. There are those
who are overseas - Chris and Olenka, Marc and Malar and the Smiths,
Claire and the Granjon Clan. All the the Tuckmans 
in North London apart from Jo in Guatemala, Kerry and Alberta, 
Karen in the East, (big) Phil, (other) Phil,
Hiroe, Bruce who used to be in the West, Paul and Catherine in the
centre, Vince in Cambridge, the Marchants (Pete and Jo) and Kul.
Then theres Tanveer (I won, I think?), Tristan, Dorothy, Dave, 
Wing, thanks for the coffee Steve, and Rosa in Madrid ... again! 
Thanks to everyone ... !

Finally, I thank my family for the support over the years, and for
coming over now and then to visit... This thesis is dedicated to
my parents.


